Neural Networks for Joint Sentence Classification in Medical Paper Abstracts

Existing models based on artificial neural networks (ANNs) for sentence classification often do not incorporate the context in which sentences appear, and classify sentences individually. However, traditional sentence classification approaches have been shown to greatly benefit from jointly classifying subsequent sentences, such as with conditional random fields. In this work, we present an ANN architecture that combines the effectiveness of typical ANN models to classify sentences in isolation, with the strength of structured prediction. Our model achieves state-of-the-art results on two different datasets for sequential sentence classification in medical abstracts.

==> datasets.tex <==
\begin{table} [H]
\footnotesize
\centering
\setlength\tabcolsep{4.0pt}
\setlength{\extrarowheight}{3pt}
\setlength{\arraycolsep}{5pt}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{$|C|$} 	& \textbf{$|V|$} 	& Train & Validation & Test \\
\hline
\text{PubMed}	& 5	&	68k	& 15k (195k)	& 2.5k (33k) 	& 2.5k	(33k)	\\
\text{NICTA}		& 6		&	17k &	722 (8k)		& 77 (0.9k) 	& 200 (2k)	 \\
\hline
\end{tabular}
\caption{Dataset overview.   
$|C|$ denotes the number of classes, $|V|$ the vocabulary size. For the train, validation and test sets, we indicate the number of abstracts followed by the number of sentences in parentheses.
} \label{tab:datasets}
\end{table}

